DRC-Coder: Automated DRC Checker Code Generation Using LLM Autonomous Agent

In the advanced technology nodes, the integrated design rule checker (DRC) is often utilized in place and route tools for fast optimization loops for power-performance-area. Implementing integrated DRC checkers to meet the standard of commercial DRC tools demands extensive human expertise to interpret foundry specifications, analyze layouts, and debug code iteratively. However, this labor-intensive process, requiring to be repeated by every update of technology nodes, prolongs the turnaround time of designing circuits. In this paper, we present DRC-Coder, a multi-agent framework with vision capabilities for automated DRC code generation. By incorporating vision language models and large language models (LLM), DRC-Coder can effectively process textual, visual, and layout information to perform rule interpretation and coding by two specialized LLMs. We also design an auto-evaluation function for LLMs to enable DRC code debugging. Experimental results show that targeting on a sub-3nm technology node for a state-of-the-art standard cell layout tool, DRC-Coder achieves perfect F1 score 1.000 in generating DRC codes for meeting the standard of a commercial DRC tool, highly outperforming standard prompting techniques (F1=0.631). DRC-Coder can generate code for each design rule within four minutes on average, which significantly accelerates technology advancement and reduces engineering costs.

==> txt/introduction.tex <==

\section{Introduction}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{fig/motivation.pdf}
% \vspace{-5mm}
\caption{
Comparison of traditional and automated approaches for DRC coding. 
The traditional method involves manual interpretation of design rules, manual coding, and iterative validation using Calibre reports.
The automated approach leverages LLMs for design rule interpretation, automatic code generation, and validation through code evaluation, aiming to reducing engineering costs and turnaround times.
% The traditional technology migration process involves manually converting the foundry's technology document into a DRC checker code to validate against the DRC reports from the Calibre industrial tool. 
% The proposed automated approach leverages LLMs to generate the DRC checker code from the technology document, with validation and iterative refinement through queries.
}
\label{fig:motivation}
% \vspace{-3mm}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{fig/technology_roadmap.pdf}
% \vspace{-5mm}
\caption{TSMC's technology roadmap~\cite{tsmctechroadmap}.
}
\label{fig:tech_roadmap}
% \vspace{-3mm}
\end{figure}


\iffalse
\begin{table} [t]
    \centering
    \caption{
    DRC runtime comparison between commercial EDA tool Calibre\textsuperscript{\textregistered} and grid-based DRC checker. 
    }
    \vspace{-.1in}
    \label{tab:example run time}
    \begin{tabular} { | c | c | }
        \hline 
        DRC method & Runtime \\
        \hline\hline
        Calibre\textsuperscript{\textregistered} & 215 sec \\
        \hline
        Grid-based DRC checker & 0.05 sec  \\
        \hline
    \end{tabular}
    % \vspace{-.2in}
\end{table}
\fi

\blue{Target on general Router, then NVCell is a case study}

In the era of advanced technology nodes, design technology co-optimization (DTCO) have become crucial for maintaining the pace of Moore's Law and achieving performance, power, and area (PPA) targets. A key of the success in DTCO is the automation of standard cell design, which enables rapid exploration and optimization of cell architectures. NVCell~\cite{ren2021nvcell, ho2023nvcell}, a reinforcement learning-based standard cell layout tool, exemplifies this trend by automating the design process for advanced technology nodes.

In standard cell design, design rule checking (DRC) is a critical step to ensure that layouts adhere to manufacturing constraints. 
The semiconductor industry currently relies on commercial tools like Calibre\textsuperscript{\textregistered} as the sign-off standard of DRC. 
While providing comprehensive DRC on physical coordinates, this tool is very time-consuming, which significantly slow down the design optimization cycle when rapid iterations are needed.
For instance, Calibre takes about 215 seconds to finish DRC on a standard cell with 22 devices.

To support efficient standard cell design automation, NVCell develops a fast and built-in DRC checker to accurately replicate Calibre's behavior in physical coordinates to grid domain. 
This checker operates on a grid-based layout format, which represents layout elements as coordinates on a grid (e.g., (0, 3, M0), (1, 3, M0), (2, 3, M0)). 
This is because NVCell perform placement and routing (P\&R) in the grid-based fashion (on-track).
By leveraging this simplified representation, NVCell's grid-based DRC checker can perform rapid checks on grid coordinates, providing quick feedback for the P\&R tool to optimize layouts.
NVCell can complete the DRC check of a cell with 22 devices in just 0.05 seconds, significantly accelerating design iterations for cell layout optimization.

However, the development of the built-in DRC checker faces several challenges, as shown in Figure~\ref{fig:motivation}. 
First, engineers need to interpret complex design rule conditions based on the visual and text illustrations in the foundry-provided document.
Second, they need to manually check the matching between the checker's reports and Calibre reports and iteratively refine the DRC code.
Finally, they require to rewrite code when facing new technology nodes or foundries.
With the rapid advancement of technology nodes (e.g., TSMC's technology roadmap in Figure~\ref{fig:tech_roadmap}), these challenges result in high engineering costs and long turnaround times during technology migration.
Inspired by this, automating the DRC checker coding process is necessary for increasing the efficiency of technology migration. 

\iffalse
However, the effectiveness of layout tools heavily relies on accurate and fast feedback from ruled-based design rule checking (DRC) tools. 
As technology nodes continue to advance rapidly, engineers face a significant challenge in technology migration: rewriting the rule-based DRC checker (called Sticks).
While industrial tool Calibre serves as black-box DRC checkers, engineers must write their own DRC checker code to meet Calibre's requirements for the target technology node. 
This process also necessitates coordinate conversion due to the difference between NVCell's grid-based system and Calibre's real-world coordinates.
Thus, writing the DRC checker requires large engineering effort.
Inspired by this, automating the DRC checker generation is necessary for increasing the efficiency and effectiveness of technology migration. 
\fi

Nowadays, large language models (LLMs)~\cite{radford2019language, raffel2020exploring, chung2022scaling, nijkamp2023codegen2} have demonstrated remarkable reasoning and code generation capabilities, making them a promising solution for automating the generation process of DRC codes. 
In addition, vision language models (VLMs)~\cite{zhang2024vision} have been shown to effectively perform image reasoning.
Thus, the ability of LLMs and VLMs to generate code and understand images aligns well with the requirements of DRC code automation, including interpreting design rules based on image and text-based content and DRC code generation.

Moreover, LLMs have shown great potential in solving complex tasks through LLM autonomous agent (LLM-agent) approaches~\cite{wang2024survey}. 
In LLM-agent, LLM acts as an intelligent controller that decomposes the overall task into subtasks, generates intermediate instructions or action plans, and provides feedback and guidance. 
The key of LLM-agent is to let LLM interact with external environment like calling some utility functions to help solving problems.
By incorporating LLM-agent, the DRC code generation can benefit from 
domain-specific utility functions to enable auto-debugging for DRC code.
% iterative refinement, where the agent can provide feedback and guidance to the LLM, enabling it to improve the generated DRC checker code over multiple iterations. 

% To tackle with extensive dataset that contains large amount of layouts, it is important to design a proper information retrieval strategy.
% Techniques like Retrieval Augmented Generation (RAG) can enhance the LLM's generation capabilities by enabling efficient retrieval and integration of relevant information from various sources, including previous DRC checker code, foundry documentation, and standard cell layouts with DRC errors.

% \begin{figure*}[t]
% \centering
% \includegraphics[width=0.85\linewidth]{fig/overall flow.pdf}
% % \vspace{-5mm}
% \caption{The overall flow of our framework for automated DRC checker generation. We take Sticks code of various technology nodes and DRV layouts as inputs. The DRC reports are provided by the industrial tool Calibre, so we need to transform the coordinates into the coordinate system of Sticks reports. Then, we use LLM-agent-based framework to provide feedback to modify generated Sticks codes for our target advanced technology node. We need our Sticks DRC reports to match Calibre DRC reports.
% }
% \label{fig:flow}
% % \vspace{-3mm}
% \end{figure*}

\blue{
In this work, we propose DRC-Agent, an automated DRC code generation system using LLM-agent. 
In detail, we develop a multi-agent framework equipped with multi-modal vision capability to perform design rule interpretation and DRC code generation based on foundry-provided design rule description.
}
\red{Need to talk about the challenges of absorbing multi-modal information from design rule description and layouts. Also, why we use multi-agent for code generation, because directly generate code in one steps is too hard and unstable for LLM (still considering how to say this in this paragraph)}

% In this work, we propose an automated DRC checker generation framework that leverages the reasoning and generation capabilities of large language models (LLMs). The framework utilizes the following input materials: (1) example DRC checker code from previous technology nodes, (2) foundry-provided technology documentation describing the design rules, and (3) standard cell layouts with known DRC errors for the target technology node. The LLM, augmented by various techniques, aims to extract and generate DRC checker code for each design rule from these input sources. The overall framework is illustrated in Figure~\ref{fig:flow}.

The contribution can be summarized as follows:
\begin{itemize}
\item We are the first work for automating the DRC coding process, significantly accelerating technology migration process and reducing engineering efforts.
\item We design an LLM-agent framework that incorporates automated debugging and feedback mechanisms, enabling iterative optimization of the generated DRC checkers. \blue{multi-modality}
\item We propose several utility functions for LLMs to leverage, including vision explainer for design rule and layout, and auto-verification of generated DRC checkers.
\item Evaluation using sub-3nm technology node show that our DRC-Agent successfully generates correct DRC codes (F1 score=1.0) for all design rules considered in NVCell, while standard prompting only produce unsatisfied results (F1=0.58).
\end{itemize}
% By automating the time-consuming and error-prone process of translating foundry documentation into DRC checkers compatible with industrial tools, our framework streamlines the technology migration workflow, reducing engineering efforts and ensuring accurate DRC checking for advanced technology nodes.

\blue{Our framework can have a potential on DRC checking related problems, such as DRC document explainer, test pattern generation, etc.}

